Equivariant Neural Functional Networks for Transformers

This paper systematically explores neural functional networks (NFN) for transformer architectures. NFN are specialized neural networks that treat the weights, gradients, or sparsity patterns of a deep neural network (DNN) as input data and have proven valuable for tasks such as learnable optimizers, implicit data representations, and weight editing. While NFN have been extensively developed for MLP and CNN, no prior work has addressed their design for transformers, despite the importance of transformers in modern deep learning. This paper aims to address this gap by providing a systematic study of NFN for transformers. We first determine the maximal symmetric group of the weights in a multi-head attention module as well as a necessary and sufficient condition under which two sets of hyperparameters of the multi-head attention module define the same function. We then define the weight space of transformer architectures and its associated group action, which leads to the design principles for NFN in transformers. Based on these, we introduce Transformer-NFN, an NFN that is equivariant under this group action. Additionally, we release a dataset of more than 125,000 Transformers model checkpoints trained on two datasets with two different tasks, providing a benchmark for evaluating Transformer-NFN and encouraging further research on transformer training and performance.

==> sections/revision.tex <==
\section{\textcolor{blue}{Experiment on augmented AGNews-Transformers dataset}}

{\color{blue}
\paragraph{Experiment Setup} In this experiment, we evaluate the performance of Transformer-NFN on the AGNews-Transformers dataset augmented using the group action $\mathcal{G}_\mathcal{U}$. We perform a 2-fold augmentation for both the train and test sets. The original weights are retained, and additional weights are constructed by applying permutations and scaling transformations to transformer modules. The elements in $M$ and $N$ (see Section~\ref{subsec:group_action}) are uniformly sampled across $[-1, 1]$, $[-10, 10]$, and $[-100, 100]$.

\paragraph{Results} The results for all models are presented in Table~\ref{tab:augmented_agnews}. The findings demonstrate that Transformer-NFN maintains stable Kendall’s $\tau$ across different ranges of scale operators. Notably, as the weights are augmented, the performance of Transformer-NFN improves, whereas the performance of other baseline methods declines significantly. This performance disparity results in a widening gap between Transformer-NFN and the second-best model, increasing from 0.031 to 0.082.

\begin{table}[h]
\color{blue}
\centering
\caption{\textcolor{blue}{Performance measured by Kendall's $\tau$ of all models on augmented AGNews-Transformers dataset using the group action $\mathcal{G}_\mathcal{U}$. Uncertainties indicate standard error over 5 runs.}}
\label{tab:augmented_agnews}
\begin{tabular}{lcccc}
    \toprule
    \centering
     &  Original & $[-1, 1]$ & $[-10, 10]$ & $[-100,100]$  \\
    \midrule
    XGBoost & $0.859 \pm 0.001$ & $0.799 \pm 0.003$ & $0.800 \pm 0.001$ & $0.802 \pm 0.003$ \\
    LightGBM & $0.835 \pm 0.001$ &  $0.785 \pm 0.003$ & $0.784 \pm 0.003$ & $0.786 \pm 0.004$\\
    Random Forest & $0.774 \pm 0.003$ & $0.714 \pm 0.001$ & $0.715 \pm 0.002$ & $0.716 \pm 0.002$\\
    MLP & $\underline{0.879 \pm 0.006}$ & $\underline{0.830 \pm 0.002}$ & $\underline{0.833 \pm 0.002}$ & $\underline{0.833 \pm 0.005}$ \\
    STATNN & $0.841 \pm 0.002$ & $0.793 \pm 0.003$ & $0.791 \pm 0.003$ &  $0.771 \pm 0.013$ \\
    Transformer-NFN & $\mathbf{0.910 \pm 0.001}$ & $\mathbf{0.912 \pm 0.001}$ & $\mathbf{0.912 \pm 0.002}$ & $\mathbf{0.913 \pm 0.001}$ \\
    \midrule
    Gap & $0.031$ & $0.082$ & $0.079$ & $0.080$ \\
    \bottomrule
\end{tabular}
\end{table}

The general decline observed in baseline models highlights their lack of symmetry. In contrast, Transformer-NFN's equivariance to $\mathcal{G}_\mathcal{U}$ ensures stability and even slight performance improvements under augmentation. This underscores the importance of defining the maximal symmetric group, to which Transformer-NFN is equivariant, in overcoming the limitations of baseline methods.

\section{Computation Complexity of Equivariant and Invariant Layers}
The computational complexity of the Transformer-NFN is derived from its invariant and equivariant layers as outlined in their pseudocode (Appendix~\ref{appendix:pseudocode_equivariant},~\ref{appendix:pseudocode_invariant}):

\begin{itemize}
    \item \textbf{Equivariant Layer Complexity:} $\mathcal{O}(d \cdot e \cdot h \cdot D^2 \cdot \max(D_q, D_k, D_v))$
    \item \textbf{Invariant Layer Complexity:} $\mathcal{O}(d \cdot e \cdot D' \cdot D \cdot \max(D \cdot h, D_A))$
\end{itemize}

Where the parameters follow our notation in Table~\ref{appendix:dimensions}.

The Transformer-NFN implementation leverages optimized tensor contraction operations (e.g., \texttt{einsum}), enabling efficient and highly parallelizable computations on modern GPUs. This ensures computational practicality while delivering significant performance improvements.
}

